Large-scale Pre-trained Models are Surprisingly Strong in Incremental Novel Class Discovery

Discovering novel concepts in unlabelled datasets and in a continuous manner is an important desideratum of lifelong learners. In the literature such problems have been partially addressed under very restricted settings, where novel classes are learned by jointly accessing a related labelled set (e.g., NCD) or by leveraging only a supervisedly pre-trained model (e.g., class-iNCD). In this work we challenge the status quo in class-iNCD and propose a learning paradigm where class discovery occurs continuously and truly unsupervisedly, without needing any related labelled set. In detail, we propose to exploit the richer priors from strong self-supervised pre-trained models (PTM). To this end, we propose simple baselines, composed of a frozen PTM backbone and a learnable linear classifier, that are not only simple to implement but also resilient under longer learning scenarios. We conduct extensive empirical evaluation on a multitude of benchmarks and show the effectiveness of our proposed baselines when compared with sophisticated state-of-the-art methods. The code is open source.

==> utils/my_acronym.tex <==
% ======================================================================================================
% My Acronym
% ======================================================================================================
% \newacronym{}{}{}
\newacronym{ai}{AI}{Artificial Intelligence}
\newacronym{ncd}{NCD}{Novel Class Discovery}
\newacronym{cincd}{class-iNCD}{class-incremental Novel Class Discovery}
\newacronym{cincdwosl}{class-iNCDwoSL}{class-incremental Novel Class Discovery without supervised learning}

\newacronym{dc}{DC}{Deep Clustering}
\newacronym{il}{IL}{Incremental Learning}

\newacronym{newsetting}{class-iNCDwoSPT}{class-incremental Novel Class Discovery without Supervised Pre-Training}

